Predicting the Spatially Varying Infection Risk in Indoor Spaces Using an Efficient Airborne Transmission Model

We develop a spatially dependent generalisation to the Wells-Riley model and its extensions applied to COVID-19, that determines the infection risk due to airborne transmission of viruses. We assume that the concentration of infectious particles is governed by an advection-diffusion-reaction equation with the particles advected by airflow, diffused due to turbulence, emitted by infected people and removed due to the room ventilation, inactivation of the virus and gravitational settling. We consider one asymptomatic or presymptomatic infectious person who breathes or talks, with or without a mask and model a quasi-3D setup that incorporates a recirculating air-conditioning flow. A semi-analytic solution is available and this enables fast simulations. We quantify the effect of ventilation and particle emission rate on the particle concentration, infection risk and the `time to probable infection' (TTPI). Good agreement with CFD models is achieved. Furthermore, we derive power laws that quantify the effect of ventilation, emission rate and infectiousness of the virus on the TTPI. The model can be easily updated to take into account modified parameter values. This work paves the way for establishing `safe occupancy times' at any location and has direct applicability in mitigating the spread of the COVID-19 pandemic.

==> Round1/former-methodology.tex <==
\subsection{The Governing Equation}

In our model, the governing equation  for the airborne transmission of COVID-19 is the advection--diffusion equation
\begin{equation} \label{eq:adv-diff-eq} \frac{\partial C}{\partial t} = \nabla \cdot (K \nabla C) - \nabla \cdot (\vec{v} C) + S, \end{equation}
where $C$ is the concentration of airborne infectious particles (particles/m$^3$), $t$ is time (s), $K$ is the isotropic diffusion coefficient of the particles in air (m$^2$/s), \ian{Is this the right terminology? I would have thought this meant molecular diffusivity rather than eddy diffusivity.} $\vec{v}$ is the advection velocity (m/s), and $S$ is the sum of sources and sinks of viral particles \cite{transport}.
% $S$ is the local source or sink contribution

In indoors locations, advection of the viral particles is due to air conditioning. We assume that the recirculation of air leads to turbulent mixing and hence turbulent diffusion of the infectious particles. Therefore, the airborne particles carrying SARS-CoV-2 diffuse and are transported by the airflow. %We will use the advection--diffusion equation to study the airborne transmission of SARS-CoV-2 with quick explorations.

\subsection{Model Assumptions}
We will apply the advection--diffusion equation in two-dimensions to study airborne transmission of COVID-19 indoors. All parameters and their values are found in Table \ref{tab:parameters}.

We follow \cite{Khalid2020} and model the source of the infectious particles, the infected person who is breathing or talking, as a continuous point source emitting viral particles at a constant rate of $R$ particles/s. Thus, a person speaking or breathing at position ($x_0$,$y_0$) starting at time $t=t_0$ \ian{looks a bit funny to say begins breathing at $t_0$. We should probably clarify that this is in some sense our start time but before this not much has happened.}
\zechariah{is it better to just drop $t_0$ then?}
\ian{No, let's keep it. I will just rephrase this.}
will be modelled as follows:
\begin{equation} \label{eq:source} S = R \delta(x-x_0) \delta(y-y_0) H(t-t_0), \end{equation}
where $\delta(x)$ is the Kronecker delta function and $H(t)$ is the Heaviside step function.

At the time of this work, $R$ is still unknown. We make the simplifying assumption that every airborne respiratory particle produced contains the virus. In other words, the emission rate of airborne virus-carrying particles, $R$, is the same as the average emission rate of airborne respiratory particles.

Following \cite{Drivas1996} we model the ventilation in the room as a sink term of uniform strength over the domain,
\begin{equation} \label{eq:vent} S_{vent} = - \lambda C, \end{equation}
where $\lambda$ is the air exchange rate of the room, measured in s$^{-1}$. We note that this is an approximation since removal of the air by ventilation occurs at a higher rate near the outlet \cite{Shao2017}. However, this method allows us to include the effect of ventilation while retaining the key features and without greatly increasing the mathematical complexity of our model.

We assume that the droplets due to breathing and talking are released from the infected person with zero initial velocity. Therefore, the advection velocity of the airborne particles, $\vec{v}$, depends solely on the airflow velocity, which, in turn, is solely controlled by the air conditioning unit.

As $\vec{v}$ is small (see Table \ref{tab:parameters} for typical values) compared to the speed of sound (340 $\rm {m/s}$), we assume that the air is an incompressible fluid \cite{Acheson}. Hence, the corresponding mass conservation equation is
\begin{equation} \label{eq:incompressible-fluid} \nabla \cdot \vec{v} = 0. \end{equation} 

We substitute equations \eqref{eq:source} assuming there is only one infectious person in the domain, \eqref{eq:vent} and \eqref{eq:incompressible-fluid} into the advection--diffusion equation \eqref{eq:adv-diff-eq} to obtain the partial differential equation (PDE) we will be working with
\begin{equation} \label{eq:basePDE} \frac{\partial C}{\partial t} + \vec{v}\cdot(\nabla C) - K \nabla^2 C = R \delta(x-x_0) \delta(y-y_0) H(t-t_0) - \lambda C.  \end{equation}

To take into account the turbulent mixing, we apply the turbulent eddy diffusion model \cite{Nicas2009}, in which $K$ is governed by the isotropic eddy diffusion coefficient. The eddy diffusion coefficient describes how quickly particles disperse with time due to turbulent mixing indoors, which occurs much more rapidly than molecular diffusion due to Brownian motion. 

At the time of writing the second wave of the pandemic had hit several countries who were debating whether it was safe to reopen schools and universities for face-to-face teaching. Hence, we decided to simulate an average classroom of dimensions 8m ($l$) $\times$ 8m ($w$) $\times$ 3m ($h$). The schematics of this room may be seen in Figure \ref{fig:schematic}. For this classroom, we assume that the airflow from the air conditioning unit is constant and uniform. Therefore, $\vec{v}$ = ($v,0$), with $v$ constant.
\zechariah{Changed schematics - 11/11/2020; changed font with overpic - 16/11/2020}
\begin{figure}[H]
\begin{center}
\begin{overpic}[width=.5\textwidth,tics=10]{Schematic.png}
\put(46,98){8m}
\put(-5,50){8m}
\put(40,65){$v$ = 0.15m/s}
\put(80,0){Air vent}
\put(20,38){Infectious person (4,4)}
\put(52,52){Position A (5,4)}
\put(54,85){Position B (8,8)}
\end{overpic}
\caption{Schematic of the modelled room.}
\label{fig:schematic}
\end{center}
\end{figure}

We consider four values of $\lambda$, the air exchange rate, corresponding to the following four ventilation settings:
\begin{enumerate}
    \item No ventilation
    \item Poor ventilation
    \item A pre-pandemic recommended ventilation setting
    \item A pandemic-updated recommended ventilation setting 
\end{enumerate}
With no ventilation $\lambda = 0$. For the poor ventilation scenario, we use the mean value for a closed classroom with the air conditioning on from an Australian primary school study by \cite{Guo2008} that investigated the impact of air exchange rates on the indoor pollution particle number concentration.
For the last two scenarios, we consider the recommended air exchange rate for classrooms made by the American Society of Heating, Refridgeration and Air-Conditioning Engineers' (ASHRAE) pre-pandemic \cite{ASHRAE-rec} and their current pandemic-updated recommendation \cite{web:ASHRAE-rec2}, respectively.

To determine an (approximate) $K$, we use the following formula for the eddy diffusion coefficient in an isothermal room `served by mixing ventilation'
%via supply and exhaust vents in the ceiling 
developed by \cite{Foat2020} which is based on the turbulent kinetic energy balance (TKEB) relationship initially proposed by \cite{Karlsson1994}:
\begin{equation} \label{eq:TKEB} K = c_v Q (2c_{\epsilon} V N^2)^{-1/3}. \end{equation}
Here $c_v$ is the von Karman constant, $Q$ is the total volume flow rate into the room, $V$ is the volume of the room, $N$ is the number of air supply vents, and $c_{\epsilon}$ is the constant of proportionality in Taylor's Dissipation Law \cite{Karlsson1994,Taylor1935}. As $Q = V \times \lambda$, \eqref{eq:TKEB} may be rewritten as
\begin{equation} \label{eq:K} K = c_v V \lambda (2c_{\epsilon} V N^2)^{-1/3}.  \end{equation}
As this formula for $K$ requires that $\lambda > 0$, for our no ventilation case, we calculated the associated $K$ assuming a low $\lambda$ of value 0.12 h$^{-1} \approx 3.3 \times 10^{-5} \mathrm s^{-1}$, which we derived from the work of \cite{Guo2008}.

We note that there is some uncertainty about the value of $c_{\epsilon}$. \cite{Karlsson1994} assumed that $c_{\epsilon} = c_v^3 = 0.032$ \cite{Bodin1979}, using an older value of $c_v = 0.32$  \cite{Bodin1979}. However, when \cite{Drivas1996} and \cite{Foat2020} applied the TKEB formula, they used a different formula for $c_{\epsilon}$; \cite{Drivas1996} used $ c_{\epsilon} = c_v = 0.4$ without providing a rationale, while \cite{Foat2020} used $c_{\epsilon} = 0.032$, citing the value used in \cite{Karlsson1994} without realising that due to the different value of $c_v$, they were using a different formula of $c_{\epsilon} = 0.5 c_v^3$. Finally, \cite{Puga2017} measured $c_{\epsilon}$ = 0.87, for sufficiently high values of Taylor Reynolds number. In this paper, we assume the formula of $c_{\epsilon} = c_v^3$ following \cite{Karlsson1994,Bodin1979} and hence have $c_{\epsilon} = 0.0593$.

We will also consider an infectious person wearing a face mask. The efficiency of surgical face masks and N95 respirators are well-documented \cite{Li2006}. However, due to the sudden demand produced by a global pandemic, there is a shortage of such masks. Many people have had to make do with cloth face masks. The efficiency of these masks is not well studied; at the moment there is only a preliminary study by \cite{Fischer2020}, which suggests that the efficiency is at least 50\%. Furthermore, a fraction of the general public wear their face masks incorrectly, which reduces their efficiency. Thus, we assume that a mask has an efficiency of 50\% (the worst-case scenario).

\begin{table}[H]
\centering
\begin{tabular}{|p{1in}|c|p{2.2in}|c|}
%p{1.4in}
\hline
Parameter & Symbol & Value & Source \\
\hline
 \multirow{4}{1in}{Rate of production of infectious particles} 
& & Breathing: 0.5 particle/s & \cite{Asadi2019} \\
&$R$ & Speaking: 5 particles/s & \cite{Asadi2019} \\
& & Breathing with mask: 0.25 particles/s & \cite{Fischer2020}\\
& & Speaking with mask: 2.5 particles/s & \cite{Fischer2020} \\
\hline
Airflow speed & $v$ & 0.15 m/s & \cite{ASHRAE} \\
\hline
Length of room & $l$ & 8m & \\
\hline
Width of room & $w$ & 8m & \\
\hline
Height of room & $h$ & 3m & \\
\hline
  \multirow{2}{1in}{Air exchange rate of room} & $\lambda$ & No ventilation: 0 h$^{-1}$ & \\
  & & Poor ventilation: 0.72 h$^{-1} \approx 2 \times 10^{-4}$ s$^{-1}$ & \cite{Guo2008} \\
  & & Pre-pandemic recommended ventilation: 3 h$^{-1} \approx 8.33 \times 10^{-4}$ s$^{-1}$ & \cite{ASHRAE-rec} \\
& & Pandemic-updated recommended ventilation: 6 h$^{-1} \approx 1.67 \times 10^{-3}$ s$^{-1}$ & \cite{web:ASHRAE-rec2} \\
 \hline
 von Karman constant & $c_v$ & 0.39 & \cite{Andreas2009} \\
 \hline
 Constant in Taylor's Dissipation Law & $c_{\epsilon}$ & 0.00593 & \cite{Bodin1979} \\
 \hline
 \multirow{2}{1in}{Eddy diffusion coefficient} & $K$ & No ventilation: 8.8 $\times 10^{-4}$ m$^2$/s & \cite{Foat2020}  \\
 & & Poor ventilation: 5.3 $\times 10^{-3}$ m$^2$/s & \cite{Foat2020} \\
 & & Pre-pandemic recommended ventilation: 2.20 $\times 10^{-2}$ m$^2$/s & \cite{Foat2020} \\
 & & Pandemic-updated recommended ventilation: 4.41 $\times 10^{-2}$ m$^2$/s & \cite{Foat2020} \\
 \hline
\end{tabular}
\captionof{table}{Parameter values}
\label{tab:parameters}
\end{table}

\subsection{Initial and Boundary Conditions}
\zechariah{moved dimensional solution here as discussed in our last meeting - 11/11/2020}

We assume that the initial concentration of infectious aerosols in the room is zero, and that the infected person, the source of infectious particles, is located at the centre of the room. The room walls are modelled as reflecting boundaries, so the boundary conditions are 
\begin{subequations} \label{eq:BC} \begin{align} & K \frac{\partial C}{\partial x}(0,y,t) - v_x C(0,y,t) = 0 \\
& K \frac{\partial C}{\partial x}(l,y,t) - v_x C(l,y,t) = 0 \\
& K \frac{\partial C}{\partial y}(x,0,t) - v_y C(x,0,t) = 0 \\
& K \frac{\partial C}{\partial y}(x,w,t) - v_y C(x,w,t) = 0 \end{align} \end{subequations}

We solve the PDE \eqref{eq:basePDE} with the boundary conditions \eqref{eq:BC} by first solving the homogeneous problem to determine the impulse function of the system and then we convolve this impulse with the source function \eqref{eq:source} to obtain the solution \cite{Evans}. 
When considering the homogeneous problems, the sink term may be separated by assuming a solution to the homogeneous problem of the form $\hat C = A e^{-\lambda t}$ \cite{Evans}. We then use the change of variable $\xi = x - vt$ and separation of variables to reduce the problems into one-dimensional diffusion problems \cite{Evans}. Due to the reflecting boundaries, we can use the method of images \cite{Shao2017,Crank} when solving for the impulse. Hence, the analytical solution is given by

 \begin{equation} \label{eq:indoors-sol} \begin{split} C(x,y,t) = &  \int_{0}^{t} \frac{R }{4\pi K} \sum_{m=-\infty}^{\infty} \left( e^{-\frac{(x - v_x (t-\tau) - x_0 - 2ml)^2}{4K(t-\tau)}} + e^{-\frac{(x + v_x (t-\tau) + x_0 - 2ml)^2}{4K(t-\tau)}} \right)  \times \\
& \sum_{n=-\infty}^{\infty} \left( e^{-\frac{(y - v_y (t-\tau) - y_0 - 2nb)^2}{4K(t-\tau)}} + e^{-\frac{(y + v_y (t-\tau) + y_0 - 2nb)^2}{4K(t-\tau)}} \right) \frac{e^{-\lambda (t-\tau)}}{t-\tau}  \mathrm{d}\tau. \end{split}  \end{equation}
We note that $C$ is proportional to the strength of the source, $R$. For convenience, we introduce the dimensionless parameter $\mathcal{R}=R/R_0$, where $R_0=0.5$\,particles/s is the rate of production of infectious particles when breathing. In all of our subsequent analysis we choose to measure our production rates in terms of $\mathcal{R}$ (see Table~\ref{tab:parametersfor R}).


\begin{table}[H]
\centering
\begin{tabular}{|c|c|c|}
\hline
Scenario & $R$ (particles/s) & $\mathcal{R}=R/R_0$  \\
\hline 
Breathing & 0.5 & 1 \\
Speaking & 5 & 10 \\
Breathing with mask & 0.25 & 0.5\\ 
Speaking with mask & 2.5 & 5 \\
\hline
\end{tabular}
\captionof{table}{Rates of production of infectious particles and relative rates compared with the rate of production when breathing, $R_0=0.5$\,particles/s.}
\label{tab:parametersfor R}
\end{table}
